Review of Top Quark Physics Results

As the heaviest known fundamental particle, the top quark has taken a central role in the study of fundamental interactions. Production of top quarks in pairs provides an important probe of strong interactions. The top quark mass is a key fundamental parameter which places a valuable constraint on the Higgs boson mass and electroweak symmetry breaking. Observations of the relative rates and kinematics of top quark final states constrain potential new physics. In many cases, the tests available with study of the top quark are both critical and unique. Large increases in data samples from the Fermilab Tevatron have been coupled with major improvements in experimental techniques to produce many new precision measurements of the top quark. The first direct evidence for electroweak production of top quarks has been obtained, with a resulting direct determination of $V_{tb}$. Several of the properties of the top quark have been measured. Progress has also been made in obtaining improved limits on potential anomalous production and decay mechanisms. This review presents an overview of recent theoretical and experimental developments in this field. We also provide a brief discussion of the implications for further efforts.

==> mtop/LJMbiblio.tex <==
\bibitem{CDF_template} CDF Collab. (A.~Abulencia {\sl et al.}), 
 \textit{Phys. Rev. Lett.} {\bf 96}, 022004 (2006).

\bibitem{CDF_template_2} CDF and \dzero\ Collabs. (M. Zielinski),
in \textit{Proceedings of Physics at LHC} (Cracow, Poland, 2006), 
{\bf hep-ex/0610017}.

%\bibitem{D0_Nature}  D\O\ Collab. (V. Abazov et al.),
% \textit{Nature} {\bf 429}, 638 (2004).

\bibitem{D0_ljmass_RunI}   D\O\ Collab. (S. Abachi, et al.),
 \textit{ Phys.\ Rev.\ Lett.\ } {\bf 79}, 1197 (1997);\\
  D\O\ Collab. (B. Abbott, et al.), \textit{ Phys.\ Rev.\ } D {\bf 58}, 052001 (1998).

\bibitem{D0_ljmass_RunII}  
 D\O\ Collab. (V. Abazov et al.), to appear in 
\textit{Phys. Rev.} D,{\bf hep-ex/0609053}; \\
P. Schieferdecker, Ph.D. thesis, LMU Munchen, 2005.

\bibitem{CDF_ME} CDF Collab. (E.~Brubaker),
FERMILAB-CONF-06-124-E. in \textit{Proceedings 41st Rencontres de Moriond on 
Electroweak Interactions and Unified Theories} ( La Thuile, Aosta Valley, 
Italy, March 11-18, 2006).

\bibitem{Kondo} 
K.~Kondo, Waseda University, \textit{RISE Technical Report} {\bf No.05-01} (2005), hep-ex/0508035.

\bibitem{QDLM} CDF Collab. (Abulencia, et al.), \textit{Phys. Rev.} D {\bf 73}, 092002 (2006). 

\bibitem{D0_ideogram_RunII}  
 D\O\ Collab. (V. Abazov et al.),
to be submitted to Phys. Rev. D,


\bibitem{W_Delphi} DELPHI Collab. (P.~Abreu et al.),
\textit{Eur. Phys. J.} C {\bf 2}, 581 (1998); 
\textit{Phys. Lett.} B {\bf 462}, 410 (1999);
\textit{Phys. Lett.} B {\bf 511}, 159 (2001); 
M.~Mulders, \textit{Ph.D.~thesis} (FOM, Amsterdam \&  Amsterdam U.), Sep 2001, 226pp.
%\bibitem{cdfR2alljetsMass} CDF Collab. CDF-Note-8709 (2007)


\bibitem{world}The Tevatron Electroweak Working Group for the CDF and D\O\ Collaborations, hep-ex/0603039.



==> single_top/STbiblio.tex <==

%\bibitem{STD0evidencePRL} Evidence for production of single top quarks and first measurement of $V_{tb}$, hep-ex/0612052, FERMILAB-PUB-06/475-E, Submitted to PRL.
%\bibitem{STD0prdone}Multivariate searches for single top quark production   with the DZero detector, submitted to Phys. Rev. D {}, hep-ex/0604020;   Fermilab-Pub-06/069-E. 
%\bibitem{STstmc}E.E. Boos et al., Phys. Atom. Nucl. 69, 1317 (2006).

%\bibitem{STcomphep} E.~Boos {\sl et al.} [{C\rm{omp}\sc{hep}}~Collaboration],Nucl. Instrum. Methods Phys. Res. A {\bf 534}, 250 (2004)

%\bibitem{STalpgen} M.~L.~Mangano {\sl et al.}, JHEP {\bf 0307}, 001 (2003)

%\bibitem{STpythia} T.~Sj\"{o}strand {\sl et al.}, Comput. Phys. Commun. {\bf     135}, 238 (2001).

%\bibitem{STgeant} R.~Brun {\sl et al.}, CERN Program Library Long Writeup  {\bf W5013} (1994).

%\bibitem{d0runI} B.~Abbott {\sl et al.} [Dzero Collaboration], Phys. Rev. D {\bf 63}, 031101 (2001);V.~M.~Abazov {\sl et al.} [Dzero Collaboration], Phys. Lett. B {\bf 517}, 282 (2001).

%\bibitem{STAcosta} D.~Acosta {\sl et al.} [CDF Collaboration], Phys. Rev. D {\bf 65}, 091102 (2002);  D.~Acosta {\sl et al.}  [CDF Collaboration],   Phys.\ Rev.\ D {\bf 69}, 052003 (2004).

%\bibitem{RunIIcdf_result} D.~Acosta {\sl et al.} [CDF Collaboration],Phys. Rev. D {\bf 71}, 012005 (2005).

%\bibitem{STPLBD0} V.~M.~Abazov {\sl et al.} [D0 Collaboration], Phys. Lett. B {\bf 622},(2005).

%\bibitem{STvariables} E.~Boos and L.~Dudko, Nucl. Instrum. Methods A {\bf 502}, 486 (2003).
%\bibitem{STMahlon:1995zn} G.~Mahlon and S.~Parke, Phys. Rev. D {\bf 53}, 4886 (1996);S.~Parke and Y.~Shadmi, Phys. Lett. B {\bf 387}, 199 (1996); G.~Mahlon and S.~J.~Parke, Phys.\ Rev.\ D {\bf 55}, 7249 (1997).
%\bibitem{STmlpfit} J.~Schwindling, \\ {\verb+http://schwind.home.cern.ch/schwind/MLPfit.html+}.
%\bibitem{STNNBayes} M.~Feindt, e-Print Archive physics/0402093 (2004).

%\bibitem{STNNstopping} G.~Orr and K.~M\"{u}ller,  ``Neural Networks: Tricks of the Trade,'' Springer-Verlag, Berlin, p. 55 (1998).

\bibitem{STLDisc}  M.~Narain  [\dzero\ Collaboration], published 
in the proceedings of International Europhysics Conference on High 
Energy Physics, Lisbon, Portugal, July 2005;
M~Begel  [\dzero\ Collaboration], published in the proceedings of   
International Workshop on Top Quark Physics, Coimbra, Portugal, January 2006.

%\bibitem{STmadevent}T. Stelzer and W.F. Long, Comput. Phys. Commun. {\bf 81},  337 (1994);   F. Maltoni and T. Stelzer, J. High Energy Phys. 02 (2003) 027.
\bibitem{STCDFttbarxsec} 
CDF Collaboration, D. Acosta {\it et al.}, hep-ex/0410041.

\bibitem{STCDFNN}  [CDF Collaboration], hep-ex/0610074.

%\bibitem{STdt-breiman} L.~Breiman {\it et al.}, {\it Classification and Regression   Trees} (Wadsworth, Stamford, 1984).
%\bibitem{STDTboost}Y.~Freund and R.E.~Schapire, in {\it Proceedings of the Thirteenth   International Conference on Machine Learning,} edited by L.~Saitta (Morgan Kaufmann, San Fransisco, 1996), p.~148.
%\bibitem{STFNALtalk}  [D0 Collaboration], {\it Evidence for Single Top Quark     Production and First Measurement of |$V_{tb}$|} presented on Dec 8th, 2006 at the Fermilab Joint Theory and Experimental Seminar.
%\bibitem{STbayesianNN} R.M.~Neal, {\it Bayesian Learning of Neural Networks} (Springer-Verlag, New York, 1996); Used ``Software for Flexible Bayesian Modeling'' package, {\texttt http://www.cs.toronto.edu/$\sim$radford/fbm.software.html}.

